Characterizing and Understanding Software Security Vulnerabilities in Machine Learning Libraries

The application of machine learning (ML) libraries has been tremendously increased in many domains, including autonomous driving systems, medical, and critical industries. Vulnerabilities of such libraries result in irreparable consequences. However, the characteristics of software security vulnerabilities have not been well studied. In this paper, to bridge this gap, we take the first step towards characterizing and understanding the security vulnerabilities of five well-known ML libraries, including Tensorflow, PyTorch, Sickit-learn, Pandas, and Numpy. To do so, in total, we collected 596 security-related commits to exploring five major factors: 1) vulnerability types, 2) root causes, 3) symptoms, 4) fixing patterns, and 5) fixing efforts of security vulnerabilities in ML libraries. The findings of this study can assist developers in having a better understanding of software security vulnerabilities across different ML libraries and gain a better insight into their weaknesses of them. To make our finding actionable, we further developed DeepMut, an automated mutation testing tool, as a proof-of-concept application of our findings. DeepMut is designed to assess the adequacy of existing test suites of ML libraries against security-aware mutation operators extracted from the vulnerabilities studied in this work. We applied DeepMut on the Tensorflow kernel module and found more than 1k alive mutants not considered by the existing test suits. The results demonstrate the usefulness of our findings.

==> figures_src/fig5.tex <==



\begin{center}
\begin{figure*}[t]
    \centering
     \makebox[\textwidth]{\includegraphics[width=14cm]{figure/componentsdiag.png}}
    \caption{Taxonomy of affected components in ML libraries.}
    \label{compdiag}
\end{figure*}
\end{center}


==> figures_src/fig6.tex <==

\begin{figure*}[t]
	\centering
	\renewcommand{\arraystretch}{0.5}%
	\setlength\fboxsep{0pt}
	\setlength\fboxrule{0.15pt}
	\includegraphics[width=6in]{figure/regex.png}
	\caption{An excerpt of rule we used to extract software vulnerabilities from Github}
	\label{rule}
\end{figure*}



==> table/deepMut.tex <==
\begin{table}[h]
\caption{Summary of alive mutants detected by {\tool} (SL denotes the start line and EL denotes the end line).}
\setlength{\tabcolsep}{3pt}
\label{deepmuttbl}
\centering
\scalebox{0.8}{
\begin{tabular}{lllll}
\hline
No & SL & EL & Filename                     & Tests                         \\
\hline
1  & 81         & 84          & broadcast\_to\_op.cc         & broadcast\_to\_op\_test.py         \\
2  & 53         & 56          & argmax\_op.cc                & argmax\_op\_test.py                \\
3  & 85         & 88          & concat\_op.cc                & concat\_op\_test.py                \\
4  & 294        & 294         & quantile\_ops.cc            & quantile\_ops\_test.py             \\
5  & 65         & 71          & xent\_op.cc                  & xent\_op\_test.py                  \\
6  & 52         & 56          & xent\_op.cc                  & xent\_op\_test.py                  \\
7  & 166        & 166         & tensor\_array\_ops.cc        & tensor\_array\_ops\_test.py        \\
8  & 424        & 424         & tensor\_array\_ops.cc        & tensor\_array\_ops\_test.py        \\
9  & 71         & 72          & variable\_ops.cc             & variable\_ops\_test.py             \\
10 & 100        & 100         & variable\_ops.cc             & variable\_ops\_test.py             \\
11 & 65         & 66          & transpose\_op.cc             & transpose\_op\_test.py             \\
12 & 170        & 170         & sparse\_tensors\_map\_ops.cc & sparse\_tensors\_map\_ops\_test.py \\
13 & 65         & 67          & sparse\_xent\_op.cc          & sparse\_xent\_op\_test.py          \\
14 & 68         & 73          & sparse\_xent\_op.cc          & sparse\_xent\_op\_test.py          \\
15 & 53         & 53          & sparse\_add\_op.cc           & sparse\_add\_op\_test.py           \\
16 & 71         & 71          & sparse\_add\_op.cc           & sparse\_add\_op\_test.py           \\
17 & 30         & 30          & base64\_ops.cc               & base64\_ops\_test.py               \\
18 & 43         & 43          & base64\_ops.cc               & base64\_ops\_test.py               \\
19 & 195        & 197         & conv\_ops.cc                 & conv\_ops\_test.py                 \\
20 & 754        & 754         & sparse\_cross\_op.cc         & sparse\_cross\_op\_test.py   \\
\hline
\end{tabular}
}
\end{table}

==> table/deepMuteStatistics.tex <==
\begin{table*}[h]
\caption{Statistics of Automated Mutation Testing on Tensorflow core Kernel}
\label{deepmutestatistics}
\centering
\scalebox{0.8}{
\begin{tabular}{llllll}
\hline
Operator               & \# Potential Mutants & \# applied mutants & \# Alive mutants & \# Killed Mutants & Mutation Score \\
\hline
Delete OP\_REQUIRE     & 1158                 & 578                & 483              & 95                & 0.16           \\
Delete OP\_REQUIRE\_OK & 2012                 & 983                & 824              & 159               & 0.19          \\
\hline
\end{tabular}
}
\end{table*}


==> table/table5.tex <==

% \begin{table}[h]
% \caption{Subcategories of Memory Release Management Issue}
% \label{memoryrelease}
% \setlength{\tabcolsep}{20pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ccc}
% \hline
% \multirow{}{}{Library} & \multicolumn{2}{c}{Memory Release Management Issue}                             \\
% \hline
%  & MRM$^1$ & IRM$^2$ \\
%                          \hline
% Tensorflow               & 2                                                  & 1                          \\
% PyTorch                  & 1                                                  & 0                          \\
% Sickit-learn             & 5                                                  & 0                          \\
% Pandas                   & 1                                                  & 0                          \\
% Numpy                    & 52                                                 & 5                          \\
% \hline
% Sum                      & 61                                                 & 6                   \\      
% \hline
% \end{tabular}}
% \vskip3pt
% $^1$ Missing Release of Memory after Effective Lifetime  $|$
% $^2$ Improper Release of Memory 

% \end{table}



==> table/typeComparison.tex <==
% \begin{table*}[t!]
% \centering
% \caption{Comparison of vulnerability types in ML libraries and traditional software systems}
% \label{typecomparison}
% \setlength\tabcolsep{3.0pt}
% \begin{tabular}{cccccc}
% \hline
%  & Numeric & Memory & API & Concurrency & Business Logic Errors \\
% \hline
% Ni et al. \cite{ni2020analyzing}  & yes & no  & yes & no  & yes \\
% Zhao et al. \cite{zhang2018empirical} & no  & no  & yes & no  & yes \\
% Tan et al. \cite{tan2014bug} & no  & yes & no  & yes & yes \\
% Yin et al. \cite{yin2011fixes} & no  & yes & no  & yes & yes \\
% Lu et al. \cite{lu2008learning} & no  & no  & no  & yes & no  \\
% Our work    & yes & yes & yes & yes\song{not in Fig 1} & yes \song{not in Fig 1} \\
% \hline
% \end{tabular}
% \end{table*}

\begin{table}[h]
\centering
\caption{Comparison of vulnerability types in ML libraries and traditional software systems (the entries in the table mean that either the papers characterise the corresponding vulnerabilities in the columns or not).}
\label{typecomparison}
\begin{tabular}{cccccc}
\hline
 & Numeric & Memory & API & Concurrency\\
\hline
Ni et al. \cite{ni2020analyzing}  & yes & no  & yes & no  \\
Amann et al. \cite{amann2018systematic} & no & no  & yes & no  \\
Tan et al. \cite{tan2014bug} & no  & yes & no  & yes \\
Yin et al. \cite{yin2011fixes} & no  & yes & no  & yes \\
Lu et al. \cite{lu2008learning} & no  & no  & no  & yes   \\
Our work    & yes & yes & yes & yes \\
\hline
\end{tabular}
\end{table}


